Optimal L-Systems for Stochastic L-system Inference Problems

This paper presents two novel theorems that address two open problems in stochastic Lindenmayer-system (L-system) inference, specifically focusing on the construction of an optimal stochastic L-system capable of generating a given sequence of strings. The first theorem delineates a method for crafting a stochastic L-system that has the maximum probability of a derivation producing a given sequence of words through a single derivation (noting that multiple derivations may generate the same sequence). Furthermore, the second theorem determines the stochastic L-systems with the highest probability of producing a given sequence of words with multiple possible derivations. From these, we introduce an algorithm to infer an optimal stochastic L-system from a given sequence. This algorithm incorporates advanced optimization techniques, such as interior point methods, to ensure the creation of a stochastic L-system that maximizes the probability of generating the given sequence (allowing for multiple derivations). This allows for the use of stochastic L-systems as a model for machine learning using only positive data for training.

==> test.tex <==
@inproceedings{mcquillan2018algorithms,
	title={Algorithms for inferring context-sensitive {L}-systems},
	author={McQuillan, Ian and Bernard, Jason and Prusinkiewicz, Przemyslaw},
	booktitle={Unconventional Computation and Natural Computation: 17th International Conference, UCNC 2018, Fontainebleau, France, June 25-29, 2018, Proceedings 17},
	pages={117--130},
	year={2018},
	organization={Springer}
}
@inproceedings{bernard2018inferring,
	title={Inferring stochastic {L}-systems using a hybrid greedy algorithm},
	author={Bernard, Jason and McQuillan, Ian},
	booktitle={2018 IEEE 30th International Conference on Tools with Artificial Intelligence (ICTAI)},
	pages={600--607},
	year={2018},
	organization={IEEE}
}
@book{prusinkiewicz2012algorithmic,
	title={The {a}lgorithmic {b}eauty of {p}lants},
	author={Prusinkiewicz, Przemyslaw and Lindenmayer, Aristid},
	year={2012},
	publisher={Springer Science \& Business Media}
}
@article{boyd2007tutorial,
	title={A tutorial on geometric programming},
	author={Boyd, Stephen and Kim, Seung-Jean and Vandenberghe, Lieven and Hassibi, Arash},
	journal={Optimization and engineering},
	volume={8},
	pages={67--127},
	year={2007},
	publisher={Springer}
}
@article{lindenmayer1968mathematical,
	title={Mathematical models for cellular interactions in development I. Filaments with one-sided inputs},
	author={Lindenmayer, Aristid},
	journal={Journal of {T}heoretical {B}iology},
	volume={18},
	number={3},
	pages={280--299},
	year={1968},
	publisher={Elsevier}
}

@article{prusinkiewicz1996stochastic,
	title={Stochastic {L}-systems},
	author={Prusinkiewicz, Przemyslaw},
	journal={Fractals},
	volume={4},
	number={1},
	pages={17--24},
	year={1996},
	publisher={World Scientific}
}

@book{boyd2004convex,
	title={Convex Optimization},
	author={Boyd, Stephen and Vandenberghe, Lieven},
	year={2004},
	publisher={Cambridge University Press}
}

@article{boyd2007tutorial,
	title={A tutorial on geometric programming},
	author={Boyd, Stephen and Kim, Seung-Jean and Vandenberghe, Lieven and Hassibi, Arjang},
	journal={Optimization and Engineering},
	volume={8}
}
@book{rudin1976principles,
	title={Principles of Mathematical Analysis},
	author={Rudin, Walter},
	edition={3rd},
	year={1976},
	publisher={McGraw-Hill}
}
@book{hatcher2002algebraic,
	title={Algebraic Topology},
	author={Hatcher, Allen},
	year={2002},
	publisher={Cambridge University Press}
}
@article{nishida1980k0l,
	title={K0{L}-System Simulating Almost but not Exactly the Same Development: Case of Japanese Cypress},
	author={Nishida, Taishin},
	journal={Memoirs of the Faculty of Science, Kyoto University. Series of biology. New {s}eries},
	volume={8},
	number={1},
	pages={97--122},
	year={1980},
	publisher={Faculty of Science, Kyoto University}
}
@online{algorithmicbotany,
	author = {{University of Calgary}},
	title = {Algorithmic {B}otany},
	date = {2017-05-01},
	url = {http://algorithmicbotany.org/}
}
@article{cieslak2022system,
	title={L-system models for image-based phenomics: case studies of maize and canola},
	author={Cieslak, Mikolaj and Khan, Nazifa and Ferraro, Pascal and Soolanayakanahally, Raju and Robinson, Stephen J and Parkin, Isobel and McQuillan, Ian and Prusinkiewicz, Przemyslaw},
	journal={in silico Plants},
	volume={4},
	number={1},
	pages={diab039},
	year={2022},
	publisher={Oxford University Press UK}
}
@article{ben2009survey,
	title={A survey on L-system inference},
	author={Ben-Naoum, Farah},
	journal={INFOCOMP Journal of Computer Science},
	volume={8},
	number={3},
	pages={29--39},
	year={2009}
}
@article{ubbens2017deep,
	title={Deep plant phenomics: a deep learning platform for complex plant phenotyping tasks},
	author={Ubbens, Jordan R and Stavness, Ian},
	journal={Frontiers in plant science},
	volume={8},
	pages={276225},
	year={2017},
	publisher={Frontiers}
}
@article{cieslak2022system,
	title={L-system models for image-based phenomics: case studies of maize and canola},
	author={Cieslak, Mikolaj and Khan, Nazifa and Ferraro, Pascal and Soolanayakanahally, Raju and Robinson, Stephen J and Parkin, Isobel and McQuillan, Ian and Prusinkiewicz, Przemyslaw},
	journal={\textit{in silico} Plants},
	volume={4},
	number={1},
	pages={diab039},
	year={2022},
	publisher={Oxford University Press UK}
}

@article{bernard2021techniques,
	title={Techniques for inferring context-free Lindenmayer systems with genetic algorithm},
	author={Bernard, Jason and McQuillan, Ian},
	journal={Swarm and Evolutionary Computation},
	volume={64},
	pages={100893},
	year={2021},
	publisher={Elsevier}
}
@article{bernard2023stochastic,
	title={Stochastic L-system inference from multiple string sequence inputs},
	author={Bernard, Jason and McQuillan, Ian},
	journal={Soft Computing},
	volume={27},
	number={10},
	pages={6783--6798},
	year={2023},
	publisher={Springer}
}
@inproceedings{mcquillan2018algorithms,
	title={Algorithms for inferring context-sensitive {L}-systems},
	author={McQuillan, Ian and Bernard, Jason and Prusinkiewicz, Przemyslaw},
	booktitle={Unconventional Computation and Natural Computation: 17th International Conference, UCNC 2018, Fontainebleau, France, June 25-29, 2018, Proceedings 17},
	pages={117--130},
	year={2018},
	organization={Springer}
}
@inproceedings{bernard2018inferring,
	title={Inferring stochastic {L}-systems using a hybrid greedy algorithm},
	author={Bernard, Jason and McQuillan, Ian},
	booktitle={2018 IEEE 30th International Conference on Tools with Artificial Intelligence (ICTAI)},
	pages={600--607},
	year={2018},
	organization={IEEE}
}
@book{prusinkiewicz2012algorithmic,
	title={The {a}lgorithmic {b}eauty of {p}lants},
	author={Prusinkiewicz, Przemyslaw and Lindenmayer, Aristid},
	year={2012},
	publisher={Springer Science \& Business Media}
}
@article{boyd2007tutorial,
	title={A tutorial on geometric programming},
	author={Boyd, Stephen and Kim, Seung-Jean and Vandenberghe, Lieven and Hassibi, Arash},
	journal={Optimization and engineering},
	volume={8},
	pages={67--127},
	year={2007},
	publisher={Springer}
}
@article{lindenmayer1968mathematical,
	title={Mathematical models for cellular interactions in development I. Filaments with one-sided inputs},
	author={Lindenmayer, Aristid},
	journal={Journal of {T}heoretical {B}iology},
	volume={18},
	number={3},
	pages={280--299},
	year={1968},
	publisher={Elsevier}
}

@article{prusinkiewicz1996stochastic,
	title={Stochastic {L}-systems},
	author={Prusinkiewicz, Przemyslaw},
	journal={Fractals},
	volume={4},
	number={1},
	pages={17--24},
	year={1996},
	publisher={World Scientific}
}

@book{boyd2004convex,
	title={Convex Optimization},
	author={Boyd, Stephen and Vandenberghe, Lieven},
	year={2004},
	publisher={Cambridge University Press}
}

@article{boyd2007tutorial,
	title={A tutorial on geometric programming},
	author={Boyd, Stephen and Kim, Seung-Jean and Vandenberghe, Lieven and Hassibi, Arjang},
	journal={Optimization and Engineering},
	volume={8}
}
@book{rudin1976principles,
	title={Principles of Mathematical Analysis},
	author={Rudin, Walter},
	edition={3rd},
	year={1976},
	publisher={McGraw-Hill}
}
@book{hatcher2002algebraic,
	title={Algebraic Topology},
	author={Hatcher, Allen},
	year={2002},
	publisher={Cambridge University Press}
}
@article{nishida1980k0l,
	title={K0{L}-System Simulating Almost but not Exactly the Same Development: Case of Japanese Cypress},
	author={Nishida, Taishin},
	journal={Memoirs of the Faculty of Science, Kyoto University. Series of biology. New {s}eries},
	volume={8},
	number={1},
	pages={97--122},
	year={1980},
	publisher={Faculty of Science, Kyoto University}
}
@online{algorithmicbotany,
	author = {{University of Calgary}},
	title = {Algorithmic {B}otany},
	date = {2017-05-01},
	url = {http://algorithmicbotany.org/}
}

@article{yu2021quantum,
	title={Quantum algorithm for approximating maximum independent sets},
	author={Yu, Hongye and Wilczek, Frank and Wu, Biao},
	journal={Chinese Physics Letters},
	volume={38},
	number={3},
	pages={030304},
	year={2021},
	publisher={IOP Publishing}
}
@article{ebadi2022quantum,
	title={Quantum optimization of maximum independent set using Rydberg atom arrays},
	author={Ebadi, Sepehr and Keesling, Alexander and Cain, Madelyn and Wang, Tout T and Levine, Harry and Bluvstein, Dolev and Semeghini, Giulia and Omran, Ahmed and Liu, J-G and Samajdar, Rhine and others},
	journal={Science},
	volume={376},
	number={6598},
	pages={1209--1215},
	year={2022},
	publisher={American Association for the Advancement of Science}
}




